Limited Linguistic Diversity in Embodied AI Datasets

Language plays a critical role in Vision-Language-Action (VLA) models, yet the linguistic characteristics of the datasets used to train and evaluate these systems remain poorly documented. In this work, we present a systematic dataset audit of several widely used VLA corpora, aiming to characterize what kinds of instructions these datasets actually contain and how much linguistic variety they provide. We quantify instruction language along complementary dimensions--including lexical variety, duplication and overlap, semantic similarity, and syntactic complexity. Our analysis shows that many datasets rely on highly repetitive, template-like commands with limited structural variation, yielding a narrow distribution of instruction forms. We position these findings as descriptive documentation of the language signal available in current VLA training and evaluation data, intended to support more detailed dataset reporting, more principled dataset selection, and targeted curation or augmentation strategies that broaden language coverage.

==> figures/dependency_parses.tex <==
\begin{figure}
    \centering
    \begin{subfigure}[b]{0.23\textwidth}
        \includesvg[width=\textwidth]{figures/rt_1_1_close-middle-drawer.svg}
        \caption{RT-1's\cite{brohan2023rt1roboticstransformerrealworld} most common sentence structure.}
        \label{fig:parses-rt-a}

    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.23\textwidth}
        \includesvg[width=\textwidth]{figures/scout_11_move-forward-five-feet.svg}
        \caption{SCOUT's\cite{lukin-etal-2024-scout-situated} most common sentence structure.}
    \end{subfigure}
    \vskip\baselineskip
    \begin{subfigure}[b]{0.23\textwidth}
        \includesvg[width=\textwidth]{figures/rt_1_2_pick-apple-from-white-bowl.svg}
        \caption{RT-1's\cite{brohan2023rt1roboticstransformerrealworld} second most common sentence structure.}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.23\textwidth}
        \includesvg[width=\textwidth]{figures/scout_12_take-a-picture.svg}
        \caption{SCOUT's\cite{lukin-etal-2024-scout-situated} second most common sentence structure.}
    \end{subfigure}
    \vskip\baselineskip
    \begin{subfigure}[b]{0.23\textwidth}
        \includesvg[width=\textwidth]{figures/rt_1_19_pick-pepsi-can-from-top-drawer-and-place-on-counter.svg}
        \caption{RT-1's\cite{brohan2023rt1roboticstransformerrealworld} third most common sentence structure.}
        \label{fig:parses-rt-e}

    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.23\textwidth}
        \includesvg[width=\textwidth]{figures/scout_14_turn-west.svg}
        \caption{SCOUT's\cite{lukin-etal-2024-scout-situated} third most common sentence structure.}
    \end{subfigure}
    \caption{Common dependency parses from investigated datasets.}
    \label{fig:parses}
\end{figure}
